Saliency-Aware Model Merging

Model merging aims to consolidate multiple task-specific models fine-tuned on different datasets into a unified architecture that performs cross-domain proficiency. Current data-free model merging methods often struggle to scale as they rely on simple parameter-level heuristics that ignore inter-layer dependencies and non-uniform distribution of expertise. This work proposes SA-Merging, which is built upon connectivity-based saliency formulations from structural pruning (e.g., SynFlow) and extends them to the data-free model merging setting. We define a saliency score over task vectors relative to a shared base model, and further introduce merge-aware modulation that incorporates agreement across experts to mitigate task interference. Based on this formulation, an iterative saliency-aware merging procedure progressively removes non-informative updates while preserving end-to-end connectivity. Furthermore, we extend SA-Merging to introduce rank-wise saliency decomposition for LoRAs without compromising their structural integrity. Extensive experiments on vision and language tasks demonstrate the effectiveness of our saliency-based approach, further reducing the gap between data-free and test-time adaptation methods.

==> tab/tab_overview.tex <==
\begin{table*}[t]
    \centering
    \small
    \setlength{\tabcolsep}{4pt}
        \begin{tabular}{lccccc}
        \toprule
        \multirow{2}{*}{Method}  &   \multicolumn{3}{c}{Language}   &   \multicolumn{2}{c}{Vision}  \\
         \cmidrule(lr){2-4} \cmidrule(lr){5-6}
        &   IA3  &   T5-Base    &   T5-Large    &   ViT-B/32 &   ViT-L/14   \\
        \midrule
        Individual &  71.4  &   82.8   &   88.8    &   90.5  &   94.2 \\
        Traditional MTL &  73.1 & 83.6 &  88.1 &   88.9  &    93.5   \\
        \midrule
        Weight Avg. &  - & 65.9 &  59.6 &   65.8    &   79.6    \\
        \midrule
        Fisher Merging  &  62.2 & 68.9 &  64.6 &   68.3  &     82.2   \\
        RegMean         &  58.0 & 71.2 &  73.2 &   71.8  &    83.7    \\
        \midrule
        Task Arithmetic &  63.9 & 73.2 &  73.5 &   60.4  &  83.3   \\
        Ties-Merging &  66.4 & 69.7 &  74.4 &   72.4  &     86.0   \\
        % Ties-Merging~\cite{} &  64.8 & 62.9 &  74.3 &   78.9  &     83.1    &   71.4  &   97.6    &   56.2    &   73.6   \\
        % AdaMerging~\cite{} &  64.5 & 68.1 &  79.2 &   93.8  &     87.0    &   91.9  &   97.5    &   59.1    &   80.1   \\
        % AdaMerging++~\cite{} &  66.6 & 68.3 &  82.2 &   94.2  &     89.6    &   89.0  &   98.3    &   60.6    &   81.1   \\
        % EMR-Merging~\cite{} &   75.2    &   72.8    &   93.5    &   99.5    &   96.9    &   98.1    &   99.6    &   74.4    &   88.7    \\
        % EMR-Merging~\cite{}* &   71.9    &   72.8    &   93.5    &   99.4    & 96.9 &   98.1  & 99.6    &   74.4    &   88.3\\
        % EMR-Merging~\cite{}$\dagger$ &   31.3    &   34.7    &   51.8    &   65.9    & 85.7 &   64.0  & 98.2    &   42.2    &   59.2    \\
        % Localize-and-Stitch~\cite{}* &   66.9    &   64.7    &   76.8    &   74.6    &   81.7    &   72.6    &   97.3    &   57.6    &   74.0    \\
        % Pareto Merging~\cite{} & 71.4    &   74.9    &   87.0    &   97.1    &   92.0    &   96.8    &   98.2    &   61.1    &   84.8    \\
        % Localize-and-Stitch~\cite{} &   67.2    &   68.3    &   81.8    &   89.4    & 87.9 &   86.6  & 94.8    &   62.9    &   79.9\\
        \midrule
        % Ours (Score-Intra)    &   61.7   &   61.7    &   68.2    &  71.2     & 62.2 &  50.3    &   83.3  &  45.1     &   63.0  \\
        % Ours (Mag-Intra)    &   58.8   &   63.2    &   68.2    &  71.2     & 75.7 &  67.4    &   96.6  &  45.1     &   70.2  \\
        % Ours (Score-Mag-Intra)    &   58.8   &   63.2    &   68.2    &  71.2     & 75.7 &  67.4    &   96.6  &  45.1     &   70.2  \\
        % Ours (SAMM-Ties-Score-Mean)    &   65.8   &   63.9    &   71.0    &  72.0     & 56.2 &  47.4    &   83.4  &  50.6     &   63.8  \\
        Ours + Ties-Merging    &   \bf 68.3   &   \bf 74.2    &   \bf 76.4    &  \bf 77.6     & \bf 89.1   \\
        Ours + Localize-and-Stitch    &  \bf 68.7   &  \bf 76.7    &  \bf 79.2    & \bf 80.9     & \bf 89.1   \\
        % Ours (8:15)    &   66.7   &   65.0    &   77.0    &  76.0     & 84.3 &  71.9    &   97.5  &  56.7     &   74.4  \\
        % Ours (10:15)    &   65.8   &   63.8    &   76.3    &  76.5     & 85.0 &  72.4    &   97.7  &  56.6     &   74.3  \\
        % Ours (15:15)    &   63.6   &   61.9    &   74.5    &  77.4     & 85.4 &  73.3    &   98.0  &  56.0     &   73.8  \\
        % Ours (12:8)    &   63.6   &   61.9    &   74.5    &  77.4     & 85.4 &  73.3    &   98.0  &  56.0     &   73.8  \\
        % Ours    &   58.8   &   63.2    &   69.0    &  82.5     & 75.7 &  67.4    &   96.6  &  51.2     &   70.2  \\
        \bottomrule
        \end{tabular}
    \caption{Multi-task performance when merging ViT-B/32 models on eight vision tasks.
    }\label{tab:overview}
    \end{table*}
